Non-Autoregressive Document-Level Machine Translation

Non-autoregressive translation (NAT) models achieve comparable performance and superior speed compared to auto-regressive translation (AT) models in the context of sentence-level machine translation (MT). However, their abilities are unexplored in document-level MT, hindering their usage in real scenarios. In this paper, we conduct a comprehensive examination of typical NAT models in the context of document-level MT and further propose a simple but effective design of sentence alignment between source and target. Experiments show that NAT models achieve high acceleration on documents, and sentence alignment significantly enhances their performance. However, current NAT models still have a significant performance gap compared to their AT counterparts. Further investigation reveals that NAT models suffer more from the multi-modality and misalignment issues in the context of document-level MT, and current NAT models struggle with exploiting document context and handling discourse phenomena. We delve into these challenges and provide our code at \url{https://github.com/baoguangsheng/nat-on-doc}.

==> discussion.tex <==
Bob: 当前NAT模型的研究主要在句子级别，取得了加速的同时，达到了和AT模型相当的性能。然而，实际应用中翻译主要是在文档级别上进行，需要考虑各个句子的文档上下文。文档上下文提供了额外信息，在AT模型上能够显著提升翻译效果。但在NAT模型上，还未有研究深入探讨如何利用上下文信息和实现上下文的连贯性。NAT模型产生的翻译在文档级别上是否能够保持连贯、消除歧义？NAT模型是否也能够利用上下文信息提升翻译效果？带着这些问题，我们探究了NAT模型在文档级别翻译上的挑战和机遇。

NAT模型面对的挑战主要来自两个问题：multi-modality和misalignment问题。句子级别上如何解决这些问题。。。然而，在文档级别上有新的挑战。。。

在这篇文章中，我们做了两件事。首先，我们评估了已有NAT模型在文档翻译上的表现，探究了面对的挑战。然后，我们提出了改进。。。


Hao: 我觉得NAT+DLMT这个想法挺好的，不过有几点concern：
1）现在的writing 稍微有点乱，直接快速读完abs和intro 可能不能掌握住重点。比如我好像没有一眼发现为啥要NAT for DLMT？后面看表格发现速度快了30倍？但是NAT速度快这个优势可能不被很多人承认，别人可能会问你们这个是在batch decoding的时候算出来的嘛？我们之前写了不少NAT的paper 其实都在claim NAT潜在未来效果更好，有bidirectional context。现在的writing NAT以及DLMT好像有点割裂。
2）方法部分，花了单独一章在介绍NAT的一些基线，后面又是一章在介绍NAT+group attention，感觉有点重复。也有点把自己的贡献打散了。我在想，这个paper 主要要claim的contribution是啥？如果是nat in DLMT，那可能就得融合起来写，写成一个，把你的方法写的non-trivial。如果是claim nat for DLMT潜力无限，但是现在问题很多，那就得花大的笔墨在分析上。现在好像有点啥都想要？
3）结果，表三和表四可以合并吗？来看你的效果提高了不少？不然现在表3都是和AT比，感觉差距还不老小。但是没看出你加了group attention之后的涨幅。最关键的事，很多cell里的BLEU都是个位数，或者0，这个看着有点离谱，审稿人可能会认为你其实没好好做实验。可能claim的贡献就是，nat in dlmt 有巨大速度优势，双向context也更适合dlmt这个场景？但是现在复杂度太高，简单做个group attention就能大幅度提高性能。也给出一些深刻的分析指出未来的方向？

